Zero-Shot Robustification of Zero-Shot Models

Zero-shot inference is a powerful paradigm that enables the use of large pretrained models for downstream classification tasks without further training. However, these models are vulnerable to inherited biases that can impact their performance. The traditional solution is fine-tuning, but this undermines the key advantage of pretrained models, which is their ability to be used out-of-the-box. We propose RoboShot, a method that improves the robustness of pretrained model embeddings in a fully zero-shot fashion. First, we use language models (LMs) to obtain useful insights from task descriptions. These insights are embedded and used to remove harmful and boost useful components in embeddings -- without any supervision. Theoretically, we provide a simple and tractable model for biases in zero-shot embeddings and give a result characterizing under what conditions our approach can boost performance. Empirically, we evaluate RoboShot on nine image and NLP classification tasks and show an average improvement of 15.98% on worst group accuracy, with trivial decrease in overall accuracy over several zero-shot baselines. Additionally, we demonstrate that RoboShot is compatible with a variety of pretrained and language models and propose a way to further boost performance with a zero-shot adaptation variant.

==> figs/intuitions_diagrams.tex <==
\begin{figure}
    \subfloat[\centering]{{\includegraphics[width=.6\textwidth]{figs/real_data_plot.pdf} }}%
    \subfloat[\centering]{{\includegraphics[width=.4\textwidth]{figs/main_projection.pdf} }}%
    \caption{(a) $\SYSNAME$ debiases original input embedding (left). The projected embedding (right)'s variance in the unwanted direction is reduced, and in the relevant direction increases. (b) Embedding projection. We project embeddings to the space orthogonal to the embeddings of all unwanted insights (e.g., \texttt{water} and \texttt{land}) }
    \label{fig:intuition}
\end{figure}

==> table/algorithm_all.tex <==
\begin{minipage}{0.48\textwidth}

\small
\begin{algorithm}[H]
        \caption{\textsc{$\SYSNAME$}} \label{alg:roboshot}
	\begin{algorithmic}[1]
		\STATE \textbf{Parameters:}
        Input embedding $x$, class embeddings $c^0, c^1$, harmful insight representations $v^1,\ldots, v^{S}$, helpful insight representations $u^1,\ldots, u^{R}$\\
            \FOR{$j \in \{1,2,\ldots, S\}$}
            \STATE Remove harmful insight $v^j$: set $x \leftarrow x-{\ip{x}{v^j}}/{\ip{v^j}{v^j}}v^j$
            \STATE Renormalize $x=x/\norm{x}$
            \ENDFOR

            \FOR{$k \in \{1,2,\ldots, R\}$}
            \STATE Amplify helpful insight $u_k$: set $x \leftarrow x+{\ip{x}{u^k}}/{\ip{u^k}{u^k}}u^k$

            \ENDFOR         
            \STATE $\hat{y}= \mathbbm{1}\{x^T c^0 < x^Tc^1\}$ 
            \STATE \textbf{Returns:} Robustified zero-shot prediction $\hat{y}$
	\end{algorithmic} 
\end{algorithm}

\end{minipage}
% \hfill
\begin{minipage}{0.48\textwidth}

\small
\begin{algorithm}[H]
        \caption{Label-free adaptation} \label{alg:lff}
	\begin{algorithmic}[1]
		\STATE \textbf{Parameters:}
        Input embedding matrix $X$, $\SYSNAME$ projected embedding matrix $X_R$, spurious insight representations $v$, useful insights representations $u$, class embeddings $c^0, c^1$, epoch number $e$
            \STATE Initialize $\Pi = X_{R}X^{\dagger}$
            \FOR{epoch in $1,2,\ldots, e$}
            \STATE $\Pi_{i+1} \leftarrow \argmin_{\Pi} \E_{x}[\mathcal{L}_{LFF}(\Pi_i x, u, v)] $ (Equation \ref{eq:lff_equation})
            \ENDFOR
            \STATE $\Pi \leftarrow BestValidation(\Pi_1,\cdots,\Pi_e) $
            \STATE $\hat{y}= \mathbbm{1}\{\Pi x ^T c^0 < \Pi x^Tc^1\}$ 
            \STATE \textbf{Returns:} Robustified zero-shot prediction $\hat{y}$
	\end{algorithmic} 
\end{algorithm}

\end{minipage}

==> table/finetuning_cshin.tex <==
\begin{table}[ht!]
\small
\caption{Self-training (ST) on CLIP ViT-B-32. We apply GRIP \cite{menghini2023enhancing} as a baseline of self-training.  ST (GRIP) uses zero-shot predicitons as pseudo-labels, ST (GRIP) + RS uses roboshot predictions as pseudo labels. ST (GRIP) + RS$^2$ applies \SYSNAME upon ST (GRIP + \SYSNAME). We trained for 3 epochs using top 10, 20, 30\% confident data. While it improves some cases, we can observe that pure \SYSNAME comparable performance without further training, especially for worst group.}

% 


   \label{tab:text_performance}
   \centering
   \begin{tabular}{lcccccccccc}
    \toprule
    \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{$\SYSNAME$} & \multicolumn{2}{c}{ST (GRIP)} & \multicolumn{2}{c}{ST (GRIP)+RS} & \multicolumn{2}{c}{ST (GRIP) + RS$^2$}\\ 
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}  \cmidrule(lr){8-9}
    & AVG & WG($\uparrow$) & AVG & WG($\uparrow$)& AVG & WG($\uparrow$) & AVG & WG($\uparrow$) \\
    \toprule
    \multirow{1}{*}{Waterbirds} & 82.0 & \cellcolor{blue!20}{\textbf{54.5}}  &  89.9 & 45.3 & 88.8 & 47.5 &  88.1 & 49.1 \\
     \midrule
     
    \multirow{1}{*}{CelebA}  & 84.8 & 80.5 & 97.8 & 60.8 &  89.4 & \cellcolor{blue!20}{\textbf{81.9}}  & 88.6 & 80.0 \\
    \midrule
    
    \multirow{1}{*}{PACS}  & 97.0 & \cellcolor{blue!20}{\textbf{86.3}} & 95.2 & 58.6  &  94.9 & 63.9 & 97.3 & 78.9\\
    
    \midrule
    \multirow{1}{*}{VLCS} & 76.5 & \cellcolor{blue!20}{\textbf{33.0}}  &72.0 & 11.4 & 73.1 & 13.6 &  77.5 & 30.7\\
    \bottomrule
   \end{tabular}
 \end{table}
